Augmenting Non-Collaborative Dialog Systems with Explicit Semantic and Strategic Dialog History

We study non-collaborative dialogs, where two agents have a conflict of interest but must strategically communicate to reach an agreement (e.g., negotiation). This setting poses new challenges for modeling dialog history because the dialog's outcome relies not only on the semantic intent, but also on tactics that convey the intent. We propose to model both semantic and tactic history using finite state transducers (FSTs). Unlike RNN, FSTs can explicitly represent dialog history through all the states traversed, facilitating interpretability of dialog structure. We train FSTs on a set of strategies and tactics used in negotiation dialogs. The trained FSTs show plausible tactic structure and can be generalized to other non-collaborative domains (e.g., persuasion). We evaluate the FSTs by incorporating them in an automated negotiating system that attempts to sell products and a persuasion system that persuades people to donate to a charity. Experiments show that explicitly modeling both semantic and tactic history is an effective way to improve both dialog policy planning and generation performance.

==> tables/fsm_example.tex <==
\begin{table}[!h]
\newcolumntype{b}{X}
\newcolumntype{s}{>{\hsize=.01\hsize}X}
\newcolumntype{m}{>{\hsize=.05\hsize}X}
\centering
\small
\begin{tabularx}{\linewidth}{XXX}
\toprule
Product Listing:\\
\midrule
\textbf{Listing Price:} 40\\
\textbf{Buyer's Target Price:} 36\\
\textbf{Title:} 2017 NEW Stans 24 and 26 Tubeless Tire Kit\\
\textbf{Product Description}:\\
``I have a NEW Stan's Tubeless tire Conversion kit for sale for 24 AND 26 wheels/tires. Pick up in Walnut Creek, CA in evenings"\\
\bottomrule
\end{tabularx}
\begin{minipage}{.5\linewidth}
\begin{tabularx}{\linewidth}{X|}
\toprule
With FSTs:\\
Seller (bot): S  Buyer: B\\
\end{tabularx}
\begin{tabularx}{\linewidth}{mb|}
\midrule
B: & Hello!\\
S: & Hi \\
FST: & \st{intro, 0.49}, \st{init-price, 0.19}...\\
B: & How old is your kit?\\
S: & I only had it for months. \\
FST: & \st{inform, 0.51}, \st{disagree, 0.20}...\\
B: & The price is a bit high, can you do 30? \\
S: & \textbf{I can't go that low. I could go down to 38.4.}\\
FST: & \st{propose price, 0.51}, \st{agree, 0.11}...\\
B: & How about 35?\\
& ...\\
\bottomrule
\end{tabularx}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\begin{tabularx}{\linewidth}{X}
\toprule
Without FSTs:\\
Seller (bot): S  Buyer: B\\
\end{tabularx}
\begin{tabularx}{\linewidth}{sb}
\midrule
B: & Hello!\\
S: & Hello \\
\\
B: & How old is your kit? \\
S: & It's only a year old.\\
\\
B: & The price is a bit high, can you do 30?\\
S: & \textbf{I can do that.}\\
\\
S: & $<$offer 30$>$\\
B: & $<$accept$>$\\
\bottomrule
\end{tabularx}
\end{minipage}
\begin{minipage}{.5\linewidth}
\begin{tabularx}{\linewidth}{X|}
\toprule
With FSTs:\\
Seller (bot): S  Buyer: B\\
\end{tabularx}
\begin{tabularx}{\linewidth}{mb|}
\midrule
B: & Hello!\\
S: & Hello \\
B: & How much are you looking for? \\
S: & I'm asking 40 for it.\\
B: & Can you do 30 dollars and I can pick it up?\\
S: & How about 37.6 ? \textbf{I will deliver to you.}\\
FST: & \st{negotiate side offers, 0.49} \\ 
& ...\\
\bottomrule
\end{tabularx}
\end{minipage}%
\begin{minipage}{.5\linewidth}
\begin{tabularx}{\linewidth}{X}
\toprule
With RNNs:\\
Seller (bot): S  Buyer: B\\
\end{tabularx}
\begin{tabularx}{\linewidth}{sb}
\midrule
B: & Hello!\\
S: & Hello \\
B: & How much are you looking for? \\
S: & I'm asking 40 for it.\\
B: & Can you do 30 dollars and I can pick it up?\\
S: & Can you do 37.6?\\
& ... \\
& \\
\bottomrule
\end{tabularx}
\end{minipage}
\caption{Examples of generated responses with FST and without FST.} 
\label{table:case_study}
\end{table}
